Unveiling the Physics of Neutron Stars: A 3D expedition into MAgneto-Thermal evolution in Isolated Neutron Stars with MATINS

This doctoral thesis investigates the long-term evolution of the strong magnetic fields within isolated neutron stars (NSs), the most potent magnetic objects in the universe. Their magnetic influence extends beyond their surface to encompass the magnetised plasma in their vicinity. The overarching magnetic configuration significantly impacts the observable characteristics of the highly magnetised NSs, i.e., magnetars. Conversely, the internal magnetic field undergoes prolonged evolution spanning thousands to millions of years, intricately linked to thermal evolution. The diverse observable phenomena associated with NSs underscore the complex 3D nature of their magnetic structure, thereby requiring sophisticated numerical simulations. A central focus of this thesis involves a thorough exploration of state-of-the-art 3D coupled magneto-thermal evolution models. This marks a pioneering achievement as we conduct, for the first time, the most realistic 3D simulations to date, spanning the first million years of a NS's life using the newly developed code MATINS, which adeptly accounts for both Ohmic dissipation and Hall drift within the NS's crust. Our simulations incorporate highly accurate temperature-dependent microphysical calculations and adopt the star's structure based on a realistic equation of state. To address axial singularities in 3D simulations, we employ the cubed-sphere coordinates. We also account for corresponding relativistic factors in the evolution equations and use the latest envelope model from existing literature, in addition to an initial magnetic field structure derived from proton-NS dynamo simulations. Within this framework, we quantitatively simulate the thermal luminosity, timing properties, and magnetic field evolution, pushing the boundaries of numerical modeling capabilities and enabling the performance of several astrophysical studies within this thesis.

==> frontmatter/empty.tex <==
\chapter*{}
\thispagestyle{empty} 
